Don't CWEAT It: Toward CWE Analysis Techniques in Early Stages of Hardware Design

To help prevent hardware security vulnerabilities from propagating to later design stages where fixes are costly, it is crucial to identify security concerns as early as possible, such as in RTL designs. In this work, we investigate the practical implications and feasibility of producing a set of security-specific scanners that operate on Verilog source files. The scanners indicate parts of code that might contain one of a set of MITRE's common weakness enumerations (CWEs). We explore the CWE database to characterize the scope and attributes of the CWEs and identify those that are amenable to static analysis. We prototype scanners and evaluate them on 11 open source designs - 4 system-on-chips (SoC) and 7 processor cores - and explore the nature of identified weaknesses. Our analysis reported 53 potential weaknesses in the OpenPiton SoC used in Hack@DAC-21, 11 of which we confirmed as security concerns.

==> results/dow_results_tbl_2.tex <==
%%import this into a latex document
{
\newcommand{\centered}[1]{\begin{tabular}{l} #1 \end{tabular}}
%% axis style, ticks, etc
\pgfplotsset{every axis/.append style={
                    label style={font=\scriptsize},
                    tick label style={font=\scriptsize}  
                    }}
\tikzset{%%
    add1mm/.style={%%
        execute at end picture={\path (current bounding box.north)--++(0,1mm);
        }
    }
}
\begin{table}[t]
\caption{Results for MITRE Top 25, Ranks 11-25} % (14,17-18,23-25 excluded)
\label{tbl:dow-results-2}
\renewcommand{\arraystretch}{0.1}
\resizebox{\columnwidth}{!}{%
\input{results/dow_results_tbl_2_tabular}
}
\vspace{-0.7cm}
\end{table}
}

==> section/detailed_algorithms.tex <==
\subsection{Algorithms}

\subsubsection{Scanner-1234}

\begin{algorithm}
\caption{CWE-1234 Detector}\label{alg:1234}
\begin{algorithmic}

\State Visitor1234 $v$
\State $mod\xrightarrow{}Accept(v)$
\State TRAVERSE$(mod)$
\State
\Procedure{traverse}{$ConditionalStatement$ $node$}

    \State $if\_expr \gets node.if\_expr$
    
    \If{$if\_expr.matches(lock\_kw,dbg\_kw,ops)$}
        \State $results.append( Result(if\_expr, loc) )$
    \EndIf
    
    \State TRAVERSE$(node.ElseStmt)$
    \State TRAVERSE$(node.ThenStmt)$
    
\EndProcedure


\end{algorithmic}
\end{algorithm}

CWE 1234 is detected by the strategy shown in algorithm \ref{alg:1234}. The detector takes a module node $mod$ as the input and outputs a $results$ vector that contains information about the detected weakness(es). A visitor $v$ object of type Visitor1234  is created. This means that $v$ will traverse the tree that it 'accepts' according to the custom functions defined in the Visitor1234 class. $v$ accepts $mod$ which starts the traversal of the AST with $mod$ as the root of the tree.

As the tree is traversed, if the node is of type ConditionalStatement, then the expression for the if statement is fetched as $if\_expr$. This if expression is then analyzed by checking if it matches three conditions. These conditions are the presence of a lock variable keyword from the list $lock\_kw$, presence of a debug keyword from the list $dbg\_kw$ and the presence of binary logical operators that would indicate 'overriding' such as the or operator. If these conditions are met, the $if\_expr$ is categorized as potentially vulnerable. A $Result$ object is created using the $if\_expr$ and location information (file, line), and the object is appended to the $results$ vector.
Following the analysis, the else and then statements of the ConditionalStatement are then traversed sequentially. Note that this recursive call takes care of possible nested if-else statements. 

% Do we need to illustrate the weakness in RTL?

\subsubsection{Scanner-1271}

\begin{algorithm}
\caption{CWE-1271 Detector}\label{alg:1271}
\begin{algorithmic}

% \State \textbf{Visitor1271} 
% \State \hskip1em $is\_reset\_block$
% \State \hskip1em $is\_reset\_lhs$
% \State \hskip1em $loc\_init\_sr$
% \State
% \State Vector$<SR>$ $sr\_vec$
% \State Visitor1271 $v$
% \State $mod\xrightarrow{}Accept(v)$
% \State TRAVERSE$(mod)$
% \State
\Procedure{traverse}{$DataDecl \: node$}
    \If{$node.IsRegisterDecl$}
        \For {$id \in node.Ids$}
        \State $n \gets id.name$
            \If{$n.m(sr\_kw) \: and \: !n.m(sr\_false\_kw)$}
            \State $sr\_vec.append(SR(n,loc))$
            \EndIf
        \EndFor
    \EndIf
\EndProcedure
\State 
\Procedure{traverse}{$ConditionalStatement \: node$}

    \State $if\_expr \gets node.if\_expr$
    
    \If{$if\_expr.matches(rst\_kw)$}
        \State $v.is\_reset\_block \gets true$
    \EndIf
    
    \State TRAVERSE$(node.ThenStmt)$
    \State $v.is\_reset\_block \gets false$
    \State TRAVERSE$(node.ElseStmt)$
    
\EndProcedure
\State
\Procedure{traverse}{$Assignment \: node$}
    \If{$v.is\_reset\_block$}
        \State $v.is\_reset\_lhs \gets true$
        \State $v.loc\_init\_sr \gets node.lval.loc$
        \State TRAVERSE$(node.lval)$
        \State $v.is\_reset\_lhs \gets false$
    \EndIf
\EndProcedure
\State
\Procedure{traverse}{$IdRef \: node$}

    \If{$v.is\_reset\_lhs$}
        \State $id \gets node.Id$
        \For{$ sr \in sr\_vec$}
            \If{$sr=id$}
                \State $sr.initialized \gets true$
                \State $sr.loc \gets v.loc\_init\_sr$
            \EndIf
        \EndFor
    \EndIf
    
\EndProcedure

\end{algorithmic}
\end{algorithm}

%1271
CWE 1271 is detected by the strategy shown in algorithm \ref{alg:1271}. A Visitor class Visitor1271 is utilized which has two boolean flags, an integer and and 4 custom functions for traversal of AST. The flag $is\_reset\_block$ is set when the tree is traversing a node which represents a reset block. The flag $is\_reset\_lhs$ is set when the tree is traversing a node that is the left hand side of an assignment inside a reset block. The integer $loc\_init\_sr$ contains the line number of the initialization of a declared identifier that is categorized as a 'sensitive register'. A class for sensitive registers, denoted as $SR$ in \ref{alg:1271}, instantiates objects $sr$ that contain information about registers that the detector classifies as 'sensitive'. These classes are illustrated in Figure~\ref{fig:1271-classes}.

A Visitor1271 object $v$ is created and accepted by the design module $mod$, in a similar manner to the 1234 detector. The traversal of the tree is dependent on the type of node.
If the node represents the declaration of some data, it is traversed according to the procedure for $DataDecl$. Here, if the declaration is of the register type. the traversal is continued, otherwise the traversal terminates for this node and returns to the parent node. If the traversal continues,m all the identifiers in the declaration item are individually analyzed. This is because a declaration may have multiple items being declared on the same line of code. If the identifier has a name that matches a keyword from $sr\_kw$ (a list containing keywords that could indicate a security relevant register) and does not match a register that contains a keyword that could be a false positive, represented in $sr\_false\_kw$, a security register object is created with the relevant information and added to the vector containing security registers.

While traversing a node that represents conditional statements, the procedure for $ConditionalStatement$ is followed. The expression for the if statement is checked for whether it could indicate a reset condition. If this condition is met, the flag for visitor indicating the traversal of a reset block - $is\_reset\_block$ is set. The statement(s) that fall within this reset block i.e. $ThenStmt$ is then traversed. After returning from this node, the $is\_reset\_block$ is set low again before traversing the else statement of the conditional statement. 
While traversing a node that represents assignments (both blocking and non-blocking), the procedure for $Assignment$ is followed. If the flag indicating this assignment is inside a reset block i.e. $is\_reset\_block$ is set high, this node is traversed, otherwise traversal terminates for this node and returns to parent node. If $is\_reset\_block$ is high, the location of the left hand assignment (line) number is assigned to the $loc\_init\_sr$ attribute of the visitor $v$. This may be used further if the left hand side contains a security sensitive register. The flag indicating a left hand side of a reset condition is set high and the left hand side of the node is traversed. On return, this flag is set low again.
While traversing a node that represents \textit{use} of declared identifiers, the procedure described in $IdRef$ is followed. These reference nodes are the terminal nodes of the tree. 
If the flag indicating this id reference is the left hand side of an assignment in a reset block i.e. $is\_reset\_lhs$ is set high, this node is traversed, otherwise traversal terminates for this node and returns to parent node. All sensitive registers in $sr\_vec$ are checked to see if they match this identifier. If there is a match, the sensitive register is marked as safe by setting its $initialized$ boolean as true and assigning a location for this initialization.

\begin{figure}[t] 
    \centering
    \includegraphics[width=0.9\linewidth]{figs/CWEAT_1271-classes.pdf}
    \caption{Classes used in 1271 scanner}
    \label{fig:1271-classes}
\end{figure}


\subsubsection{Scanner-1245}

For the CWE 1245 scanner, a few custom classes and their functionalities are utilized as shown in Figure~\ref{fig:1245-classes}. 
%  VeriScope is a symbol table of locally declared identifiers.
Objects of these classes are used in the steps below to highlight areas of weaknesses in FSMs.
\begin{enumerate}[(I)]
    \item \textit{Find FSM variables:} The scope of the module, which contains the locally declared identifiers in a symbol table, is obtained. Each of these identifiers is checked for being 'one-hot' encodable and being a variable. If these two conditions are met, it is classified as a FSM variable. All the variables are linked to this fsm variable are tracked and added to the list of variables belonging to a particular FSM i.e. \textit{state\_var\_names}. This is done to link variables like \texttt{state} with \texttt{next\_state} to represent the same FSM. This step is illustrated in algorithm \ref{alg:1245-findFSMvars}.
    \item \textit{Extract FSM transitions:} The AST of the module is traversed according the custom traversal for visitor object Visitor1245. The goal here is to collect the transitions of an FSM and adding them to the \textit{fsm} object. This step is illustrated in algorithm \ref{alg:1245-extractFSMtransitions}.
    The procedure for \textit{EventControlStatement} nodes is not algorithmically shown for brevity. It is used to enter statements of always blocks that are influenced by a 'clocked' expression. 
    % add to appendix?
    
    When traversing \textit{ConditionalStatement} nodes, the condition is checked to determine whether a state variable is being accessed. This is done by checking the operator to be the logical equality and if either the left hand side or right hand side contains an identifier that can be a FSM variable. If these conditions are met, the state variable and state information is added to the visitor object \textit{v} and the \textit{then} statement is traversed. On return, the state variable and state information is set to 0 and the \textit{else} statement is traversed. If the conditions for FSM state variable comparison are not met, the condition is pushed to the \textit{v.conditions} map and \textit{then} statement is traversed. On return the condition is popped, the \textit{else} condition is pushed to the \textit{v.conditions} map and \textit{else} statement is traversed. On return, the \textit{else} condition is popped.
    
    When traversing the \textit{CaseStatement} node, the identifier is checked. If it is an fsm variable the case statement is analyzed for completeness. This function is described in the \textit{Analyze FSM} section. Each value of each case item is then checked for a state variable comparison. If it is found, the state variable information is added to the visitor object \textit{v} and the statement for the case item is traversed. On return, the state variable information is set to 0.
    If there is no state variable comparison, the condition for case statement is pushed to the \textit{v.conditions} map before traversing case item statement.On return, the state variable information is set to 0.
    
    When traversing a \textit{Assignment} node, the assignment is determined to represent an FSM transition if the left hand side is an FSM variable adn the visitor object \textit{v} has non-zero present state information. If it is a state transition all relevant transition information is added to the \textit{fsm} object. If it is a state reset, all relevant reset information is added to the \textit{fsm} object. 
    
    \item \textit{Analyze FSM:} After all relevant information is gathered from the two previous steps, the FSM is analyzed to check for a range of weaknesses. These include unreachable state, FSM deadlock, detected through \textit{fsm.analyze\_transitions()},  and incomplete case statements, detected through \textit{v.analyze\_casestatement()}. An unreachable state is shown as \texttt{S4} in Figure~\ref{fig:fsm-weaknesses-1}; it is the initial value of a transition but there is no way to get there i.e. \texttt{S4} is not present in the final value of any transition or on reset. An FSM deadlock is shown through the dotted line leaving \texttt{S4} Figure~\ref{fig:fsm-weaknesses-1}. \texttt{S4} is the final value of a transition but there is no way to get out i.e. it is not in initial value of any transition. A case statement representing an FSM is analyzed for completeness in addition to these FSM vulnerabilities. Completeness is verified if there is either a default statement present or if the number of case items equal the possibilities from the size of case condition.
     
    
\end{enumerate}

\begin{figure}
    \begin{subfigure}{.25\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{figs/1245-fsm-weakness-1.pdf}
        \caption{Unreachable state}
        \label{fig:fsm-weaknesses-1}
    \end{subfigure}%
    \begin{subfigure}{.25\textwidth}
        \centering
        \includegraphics[width=.8\linewidth]{figs/1245-fsm-weakness-2.pdf}
        \caption{FSM deadlock}
        \label{fig:fsm-weaknesses-2}
    \end{subfigure}
    \caption{FSM weaknesses}
    \label{fig:fsm-weaknesses}
\end{figure}


\begin{figure}[t] 
    \centering
    \includegraphics[width=0.9\linewidth]{figs/CWEAT_1245-classes.pdf}
    \caption{Classes used in 1245 scanner}
    \label{fig:1245-classes}
\end{figure} 


\begin{algorithm}
\caption{CWE-1245 Detector - Find FSM variables}\label{alg:1245-findFSMvars}
\begin{algorithmic}
\State $scope \gets mod.GetScope()$ 
\For{$id \in scope.Ids$ }
    \If{$id.CanBeOneHot()\:and\:id.IsVar()$}
        \State $fsm.state\_var\_names.append(id)$
        \State $fsm.state\_var\_names.append( id.linkVars() )$
    \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{CWE-1245 Detector - Extract FSM transitions}\label{alg:1245-extractFSMtransitions}
\begin{algorithmic}
% \Procedure{traverse}{$EventControlStatement \: node$}
%     \State $v.is\_clocked \gets 0,\; sens\_list \gets node.GetAt()$
%     \For{$expr \in sens\_list$}
%         \If{$expr.IsEdge$}
%             \State $v.is\_clocked \gets 1$
%         \EndIf
%     \EndFor
%     \State $Stmt \gets node.GetStmt()$
%     \State TRAVERSE$(Stmt)$
%     \State $v.is\_clocked \gets 0$
% \EndProcedure
\Procedure{traverse}{$ConditionalStatement \: node$}
    \State $cond \gets node.IfExpr()$
    \State $then \gets node.GetThen(),\;else \gets node.getElse()$
    \If{$cond.OperType==LOGEQ)$} 
        \State $l \gets node.lhs,\;r \gets node.rhs$
        \If{$(l.isFsmVar \; or \; r.isFsmVar) $}
            \State $state\_var \gets l.isFsmVar?l:r$
            \State $v.present\_state\_var \gets state\_var.id$
            \State $v.present\_state \gets state\_var$
            \State TRAVERSE$(then)$
            \State $v.present\_state\_var \gets 0$
            \State $v.present\_state \gets 0$
            \State TRAVERSE$(else)$
        \EndIf
    \Else
        \State $v.pushCondition(cond)$
        \State TRAVERSE$(then)$
        \State $v.popCondition()$
        \State TRAVERSE$(else)$
        \State $v.popCondition()$
    \EndIf
\EndProcedure
\State \vspace{-7pt}
\Procedure{traverse}{$CaseStatement \: node$}
    \State $cond \gets node.GetCond()$
    \If{$cond.id.IsFsmVar()$}
        \State $check\_complete\_case(node)$
        \For{$case\_item \in node.CaseItems$}
            \For{$value \in case\_item.conditions$}
                \If{$!v.present\_state\_var$}
                    \State $v.present\_state \gets value$
                    \State $v.present\_state\_var \gets cond.id$
                    \State TRAVERSE$(case\_item.Stmt)$
                    \State $v.present\_state \gets 0$
                    \State $v.present\_state\_var \gets 0$
                \Else
                    \State $v.pushCondition(cond)$
                    \State TRAVERSE$(case\_item.Stmt)$
                    \State $v.popCondition()$
                \EndIf
            \EndFor
        \EndFor
    \EndIf
\EndProcedure
\State \vspace{-7pt}
\Procedure{traverse}{$Assignment \: node$}
    \If{$node.lhs.id.IsFsmVar$}
        \If{$v.present\_state$}
            \State $fsm.fsm\_transitions.append(lhs.id,$
            \State $v.present\_state,\:v.present\_state\_var,$ 
            \State $rhs.id,\: node.loc,\:v.conditions)$
        \Else
            \State
            $fsm.fsm\_state\_resets.append(lhs.id,\: rhs.id,$ 
            \State $rhs.id,\: node.loc)$
        \EndIf
    \EndIf
\EndProcedure


\end{algorithmic}
\end{algorithm}

% \begin{algorithm}
% \caption{CWE-1245 Detector - Analyze FSM}\label{alg:1245-analyzeFSM}
% \begin{algorithmic}
% \State placeholder
% \end{algorithmic}
% \end{algorithm}



\subsubsection{Scanner-1280}

\begin{figure}[t] 
    \centering
    \includegraphics[width=0.9\linewidth]{figs/CWEAT_1280-classes.pdf}
    \caption{Classes used in 1280 scanner}
    \label{fig:1280-classes}
\end{figure}  

\begin{algorithm}
\caption{CWE-1280 Detector}\label{alg:1280}
\begin{algorithmic}

%\State \textbf{Visitor1280} 
%\State \hskip1em Bool $is\_lhs$
%\State \hskip1em Bool $is\_b\_assign$
%\State \hskip1em SeqBlock $last\_block$
%\State \hskip1em Vector$<id>$ $sens\_list$
%\State \hskip1em Vector$<Tuple<id, block, lineno>>$ $reads$
%\State \hskip1em Vector$<Tuple<id, block, lineno>>$ $writes$

\Procedure{traverse}{$AlwaysConstruct \: node$}
    \State $v.sens\_list \gets node.sens\_list$
    \State TRAVERSE$(node.Stmt)$
    \State $v.sens\_list \gets [\hskip.25em]$
\EndProcedure
\State  \vspace{-5pt}
\Procedure{traverse}{$SeqBlock \: node$}
    \State SeqBlock $lastSeqB$
    \State $lastSeqB \gets v.last\_block$
    \State $v.last\_block \gets node$
    \State TRAVERSE$(node.GetStmts)$
    \State $v.last\_block \gets lastSeqB$
    
\EndProcedure
\State \vspace{-7pt}
\Procedure{traverse}{$BlockingAssign \: node$}
    \State $v.is\_b\_assign \gets True$
    \State $v.is\_lhs \gets True$
    \State TRAVERSE$(node.GetLhs)$
    \State $v.is\_lhs \gets False$
    \State TRAVERSE$(node.GetRhs)$
    \State $v.is\_b\_assign \gets False$

\EndProcedure
\State \vspace{-7pt}
\Procedure{traverse}{$IdRef \: node$}

    \If{$v.is\_b\_assign$ \textbf{and} $node.id$ \textbf{not in} $v.sens\_list$}
        \State $t \gets Id(node.id, v.last\_block, node.lineno)$
        \If{$v.is\_lhs$}
            \State $v.writes.add(t)$
        \Else    
            \State $v.reads.add(t)$
        \EndIf
    \EndIf
    
\EndProcedure
\State  \vspace{-2pt}
\Procedure{Detect\_1280}{$Module \: mod$}
    \State Visitor1280 $v$
    \State $mod.Accept(v)$
    \For{$id\_w, b\_w, lno\_w$ \textbf{in} $v.writes$}
        \For{$id\_r, b\_r, lno\_r$ \textbf{in} $v.reads$}
            \If{$id\_r=d\_w$ \textbf{and} \\ $b\_r=b\_w$ \textbf{and} \\ $lno\_r<lno\_w$}
                \State $LogCWE(1280, lno\_r, ln\o_w)$
            \EndIf
        \EndFor
    \EndFor
\EndProcedure

\end{algorithmic}
\end{algorithm}

CWE-1280 detection is based on the classes shown in Figure~\ref{fig:1280-classes}, the procedures are presented in Algorithm~\ref{alg:1280}. A Visitor class Visitor1280 is used to build two lists containing information read and write operations ($reads$ and $writes$ lists respectively) which are then analyzed to detect the CWE. Two flags, $is\_lhs$ and $is\_b\_assign$ are used to signal that the traversed node is inside a left-hand side (lhs) of an assignment and inside a blocking assign respectively. $last\_block$ keeps track of the last visited begin-end block. $sens\_list$ stores the ids of the sensitivity list of the parent always block, is an empty list if the current node does not have a parent always block. 

When traversing an always construct the visitor first copies the sensitivity list into $sens\_list$ then proceeds with the traversing of the statement. Before returning, it clears the $sens\_list$ by assigning it to an empty list.

When traversing a sequential block, the visitor stores the last visited sequential block, $v.last\_block$, in a temporary variable, $lastSeqB$, then sets $v.last\_block$ to the current node before proceeding the traversing on the block statements. before returning it restores $v.last\_block$ to the original value assigning it $lastSeqB$.

When traversing a blocking assign, the visitor sets the flags $v.is\_b\_assign$ and $v.is\_lhs$ to $True$, then it visits the lhs of the assignment. After the visit to the lhs, it sets the flag $v.is\_lhs$ to $False$ and proceeds traversing the right-hand side. Before returning it sets the flag  $v.is\_b\_assign$ to $False$.

When traversing an id reference, the visitor checks if this id is in a blocking assign and is not in the sensitivity list of the parent always block. If this condition is met, then a tuple with the information about the id is created and then added to the $writes$ list if the id is in a lhs, to the $reads$ list otherwise.

After the AST of the module has been visited and the $reads$ and $writes$ lists have been built, the detection algorithm iterates through the two lists and compare each read entry with the writes entries. If a read and a write have the same ids, are in the same begin-end block and the read comes before the write, it means that it is not reading the updated value and might be a cause of CWE-1280.
\subsubsection{Scanner-1262}
\begin{figure}[t] 
    \centering
    \includegraphics[width=0.9\linewidth]{figs/CWEAT_1262-classes.pdf}
    \caption{Class used in 1262 scanner}
    \label{fig:1262-classes}
\end{figure}
\begin{algorithm}
\caption{CWE-1262 Detector}\label{alg:1262}
\begin{algorithmic}

\State \textbf{Visitor1262} 
\State \vspace{-7pt}
\Procedure{traverse}{$AlwaysConstruct \: node$}
    \State $v.controlV \gets [\hskip.25em]$
    \State TRAVERSE$(node.Stmt)$
\EndProcedure
\State  \vspace{-5pt}
\Procedure{traverse}{$QuestionColon \: node$}
    \State $cond \gets node.IfExpr()$
    \State $then \gets node.GetThen(),\;else \gets node.getElse()$
    \State TRAVERSE$(then)$
    \State TRAVERSE$(else)$
    $v.is\_control \gets True$
    \State TRAVERSE$(cond)$
    $v.is\_control \gets False$
    
\EndProcedure
\State \vspace{-5pt}
\Procedure{traverse}{$NonBlockingAssign \: node$}
    \State $v.is\_wdata \gets False$
    \State $v.is\_rhs \gets True$
    \State TRAVERSE$(node.GetRhs)$
    \State $v.is\_rhs \gets False$
    \If{$(!v.is\_wdata)$}
        \State $return$
    \EndIf
    \State $v.is\_lhs \gets True$
    \State TRAVERSE$(node.GetLhs)$
    \State $v.is\_lhs \gets False$
\EndProcedure
\State \vspace{-5pt}
\Procedure{traverse}{$ConditionalStatement \: node$}
    \State $v.count \gets 0$
    % \State $sig\_count \gets 0$ 
    \State $cond \gets node.if\_expr$
    \State $v.is\_control \gets True$
    \State TRAVERSE$(cond)$
    \State $sig\_count \gets v.count$
    \State $v.is\_control \gets False$
    \State $then \gets node.GetThen(),\;else \gets node.getElse()$
    \State TRAVERSE$(then)$
    \State TRAVERSE$(else)$
     \For{$(i=0;i<sig\_count;i++)$}
        \State $v.controlV.pop\_back()$
      \EndFor
    \State $v.count \gets v.count-sig\_count$
    
\EndProcedure
\State \vspace{-5pt}
\Procedure{traverse}{$IdRef \: node$}

    \If{$v.is\_rhs \; and \; wdata \;in\;node.GetName()$}
        \State $v.is\_wdata \gets True$
        \State $return$
    \ElsIf{$v.is\_control$}
        \State $v.controlV.add(node.GetName()))$
        \State $count \gets count+1$
    \ElsIf{$v.is\_lhs$}    
        \State $v.sigM.add(node.GetName(),v.controlV)$
    \EndIf
\EndProcedure
\end{algorithmic}
\end{algorithm}
CWE-1262 is detected by the strategy shown in Algorithm~\ref{alg:1262}.
To detect improper access control for registers, we need to use the Visitor class Visitor1262 to build a map, which links each register to their corresponding control signals.
When traversing an always block, the visitor first builds a new array to record the control signals inside this sequential block.
Whenever the visitor finds an if/else expression, it sets $is\_control$ to True, so the visitor can push the signals inside the sensitivity list into the array.
Similar to previous other scanners, some flags are generated when the visitor is parsing assignment to differentiate the left/right-hand side values.

To narrow down the vulnerability scope, we only focus on the registers that are not properly write-protected, i.e., untrusted users could modify the value through DMA IPs.
We first traverse the right-hand side value to identify if $wdata$ exists.
If $wdata$ does not exist in the assignment, the visitor will leave this assignment as we do not need to build the map for this register.
Otherwise, a map, $sigM$ will be built to link a register value and the current control signal array, which represents all the control signals for this register specifically.
When leaving an if/else domain, the visitor needs to clear the related signals from the control signal array to ensure that protection mapping mechanism works properly.
Note that, a $count$ variable is incremented every time the visitor is traversing an if/else statement, so it records how many signals are inserted in each if/else expression.
Therefore, the visitor can pop out the associated signals from $controlV$ correctly.


After the parse tree has been analyzed and the signal protection map for each register has been built, further investigation is still required to determine which signal lacks proper control.
First, for each set of control signals, we will prune out those signals that cannot be considered ``controlling'', such as clock and reset.
After removing those irrelevant signals, if the controlling set is empty, the corresponding register is regarded as unprotected and classified as CWE-1262.

Moreover, we will also compare the control signal sets for register arrays, e.g., the $reglk\_mem$ array in Figure~\ref{fig:reglk_code}.
Since an array of signals should have the same ``level'' of protection, we compare the number of controlling signals of each to ensure that no signal is less protected.
Additionally, a warning will be raised if different entries do not have the identical group of control signals.
Since the implementation of signal protection mechanisms differs by design, some require the signal array to have the exact same set of control signals but some do not, it might not be a real vulnerability.
However, we exhibit a user exploit for this scenario in Section~\ref{xxx}.


==> section/preamble/preamblelistingsconf.tex <==
\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\makeatletter
\let\old@lstKV@SwitchCases\lstKV@SwitchCases
\def\lstKV@SwitchCases#1#2#3{}
\makeatother
\usepackage{lstlinebgrd}
\makeatletter
\let\lstKV@SwitchCases\old@lstKV@SwitchCases

\lst@Key{numbers}{none}{%
    \def\lst@PlaceNumber{\lst@linebgrd}%
    \lstKV@SwitchCases{#1}%
    {none:\\%
     left:\def\lst@PlaceNumber{\llap{\normalfont
                \lst@numberstyle{\thelstnumber}\kern\lst@numbersep}\lst@linebgrd}\\%
     right:\def\lst@PlaceNumber{\rlap{\normalfont
                \kern\linewidth \kern\lst@numbersep
                \lst@numberstyle{\thelstnumber}}\lst@linebgrd}%
    }{\PackageError{Listings}{Numbers #1 unknown}\@ehc}}
\makeatother

\usepackage{lstlinebgrd} % see http://www.ctan.org/pkg/lstaddons

\lstset{ 
%   escapeinside={(*@}{@*)},
%   backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
  basicstyle=\scriptsize,        % the size of the fonts that are used for the code
%   breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
%   captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
%   deletekeywords={...},            % if you want to delete keywords from the given language
%   escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
%   extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,	                   % adds a frame around the code
%   keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=C,                 % the language of the code
%   morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbers
%   rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
%   showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
%   showstringspaces=false,          % underline spaces within strings only
%   showtabs=false,                  % show tabs within strings adding particular underscores
%   stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
%   tabsize=2,	                   % sets default tabsize to 2 spaces
%   title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
%   %framesep=0pt,framerule=0pt,
%   %aboveskip=0pt,belowskip=0pt
}

